DFNet: Enhance Absolute Pose Regression with Direct Feature Matching

We introduce a camera relocalization pipeline that combines absolute pose regression (APR) and direct feature matching. By incorporating exposure-adaptive novel view synthesis, our method successfully addresses photometric distortions in outdoor environments that existing photometric-based methods fail to handle. With domain-invariant feature matching, our solution improves pose regression accuracy using semi-supervised learning on unlabeled data. In particular, the pipeline consists of two components: Novel View Synthesizer and DFNet. The former synthesizes novel views compensating for changes in exposure and the latter regresses camera poses and extracts robust features that close the domain gap between real images and synthetic ones. Furthermore, we introduce an online synthetic data generation scheme. We show that these approaches effectively enhance camera pose estimation both in indoor and outdoor scenes. Hence, our method achieves a state-of-the-art accuracy by outperforming existing single-image APR methods by as much as 56%, comparable to 3D structure-based methods.

==> table_tex/table4.tex <==


\begin{table}[t]
\caption{Comparison with various single-frame and sequential APR methods.}
\label{table:4}
% \renewcommand{\arraystretch}{1.2}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccc|cc}
\toprule
& PoseNet & MapNet & \makecell[c]{MapNet+\\(PGO)} & VLocNet & TransPN  & \makecell[c]{Direct-PN\\+U} & \makecell[c]{CoordiNet\\+LENS} & FNet & DFNet \\
& \cite{Kendall15,Kendall16,Kendall17} & \cite{Brahmbhatt18} & \cite{Brahmbhatt18} & \cite{Valada18} & \cite{Shavit21} & \cite{chen21} & \cite{Moreau21} & \multicolumn{2}{r}{\makecell[c]{(proposed)}}\\ %(proposed) \\
\midrule
Single-Frame APR  & \checkmark & \checkmark & $\times$ & $\times$ & \checkmark & \checkmark & $\times$ & \checkmark & \checkmark\\
Data Generation   & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & \checkmark & \checkmark & \checkmark\\
Unlabeled Training    & $\times$ & $\times$ & \checkmark & $\times$ & $\times$ & \checkmark & $\times$ & $\times$ & \checkmark\\
1-Image Optimization & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & \checkmark & $\times$ & $\times$ & \checkmark\\
\bottomrule
\end{tabular}
}
\end{table}










==> table_tex/table5.tex <==
% \begin{table}[!ht]
% \caption{Ablation on DFNet. DFM stands for Direct Feature Matching. We also show that NeRF-Hist works on photometric direct matching}
% \label{table:5}
% \centering
% \resizebox{0.4\textwidth}{!}{
%     \begin{tabular}{l|c}
%         \toprule
%         Method                               & Shop Facade \\
%         \midrule
%         FNet w/ \mathcal{L}_{triplet}^{ori}                     & 1.49m/5.80\degree  \\
%         +In-Triplet Mining                      & 1.37m/5.34\degree  \\
%         +RVS                                 & 0.72m/2.58\degree  \\
%         +DFM (NeRF-W)    & 0.43m/1.62\degree  \\
%         +DFM (NeRF-Hist) & \textbf{0.15m}/\textbf{0.65\degree}  \\
%         \midrule
%         Direct-PN                            & 1.10m/4.25\degree  \\
%         Direct-PN+U                          & 1.41m/6.97\degree  \\
%         + NeRF-Hist                          & 0.72m/3.39\degree  \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table}

% \caption{A comparison among different APR Methods}
% \label{table:4}
% \centering
% \resizebox{0.6\textwidth}{!}{
% \begin{tabular}{l|c|c|c|c}
% \toprule
% & \makecell[c]{1-frame\\Method} & \makecell[c]{Data\\Generation} & \makecell[c]{Unlabeled\\data} & \makecell[c]{Optimize\\1 image} \\
% \midrule
% Posenet      & \checkmark & $\times$ & $\times$ & $\times$ \\
% MapNet       & \checkmark & $\times$ & $\times$ & $\times$ \\
% MapNet+      & $\times$ & $\times$ & \checkmark & $\times$ \\
% TransPoseNet & \checkmark & $\times$ & $\times$ & $\times$ \\
% LENS         & $\times$ & \checkmark & $\times$ & $\times$ \\
% Direct-PN+U  & \checkmark & $\times$ & \checkmark & \checkmark \\
% Fnet (Ours)  & \checkmark & \checkmark & $\times$ & $\times$ \\
% DFNet (Ours) & \checkmark & \checkmark & \checkmark & \checkmark\\
% \bottomrule
% \end{tabular}
% }
% \end{table}

==> table_tex/table6a.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Submitted for review %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{wraptable}{r}{0.4\textwidth}

    \caption{\textbf{Feature levels vs. pose error.} We report the effect of various level of features on DFNet performance. Letter F, M, and C denote features extracted from fine, middle, and coarse levels in a VGG backboned DFNet.}
    % \vspace{0.15cm}
    \label{table:6a}
    \centering
    \resizebox{0.4\textwidth}{!}{
        \begin{tabular}{l|c}
        \toprule
        Feature Level & DFNet (ShopFacade) \\
        \midrule
        F                  & \textbf{0.15m}, \textbf{0.64°}                   \\
        F+M                & 0.19m, 0.77°                   \\
        F+M+C              & 0.20m, 0.77°                  \\
        \bottomrule
        \end{tabular}
    }

\end{wraptable}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Submitted for arXiv %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{wraptable}{r}{0.4\textwidth}
%     % \vspace{-0.7cm}
%     \caption{\textbf{Feature levels vs. pose error.} We report the effect of various level of features on DFNet performance. Letter F, M, and C denote features extracted from fine, middle, and coarse levels in a VGG backboned DFNet.}
%     % \vspace{0.15cm}
%     \label{table:6a}
%     \centering
%     \resizebox{0.4\textwidth}{!}{
%         \begin{tabular}{l|c}
%         \toprule
%         Feature Level & DFNet (ShopFacade) \\
%         \midrule
%         F                  & \textbf{0.15m}, \textbf{0.64°}                   \\
%         F+M                & 0.19m, 0.77°                   \\
%         F+M+C              & 0.20m, 0.77°                  \\
%         \bottomrule
%         \end{tabular}
%     }
% \end{wraptable}


==> table_tex/table6b.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Submitted for review %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{wraptable}{r}{0.4\textwidth}

    \caption{Ablation on DFNet (upper part) and \nerfhist in photometric direct matching (lower part). DFM denotes Direct Feature Matching.}
    \label{table:6b}
    \centering
    \resizebox{0.4\textwidth}{!}{
        \begin{tabular}{lc}
            \toprule
            Method                               & Shop Facade \\
            \midrule
            DFNet w/ $\mathcal{L}_{triplet}^{ori}$ & 1.49m/5.80\degree  \\
            +RVS                                 & 0.86m/4.05\degree  \\
            +$\mathcal{L}_{triplet}$        & 0.72m/2.58\degree  \\
            +DFM (NeRF-W)                       & 0.43m/1.62\degree  \\
            +DFM (NeRF-Hist) & \textbf{0.15m}/\textbf{0.65\degree}  \\
            \midrule
            Direct-PN                            & 1.10m/4.25\degree  \\
            Direct-PN+U                          & 1.41m/6.97\degree  \\
            + NeRF-Hist                          & 0.72m/3.39\degree  \\
            \bottomrule
        \end{tabular}
    }

\end{wraptable}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Submitted for arXiv %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{wraptable}{r}{0.4\textwidth}
%     % \vspace{-0.7cm}
%     \caption{Ablation on DFNet (upper part) and \nerfhist in photometric direct matching (lower part). DFM denotes Direct Feature Matching.}
%     \label{table:6b}
%     \centering
%     \resizebox{0.4\textwidth}{!}{
%         \begin{tabular}{lc}
%             \toprule
%             Method                               & Shop Facade \\
%             \midrule
%             DFNet w/ $\mathcal{L}_{triplet}^{ori}$ & 1.49m/5.80\degree  \\
%             +RVS                                 & 0.86m/4.05\degree  \\
%             +$\mathcal{L}_{triplet}$        & 0.72m/2.58\degree  \\
%             +DFM (NeRF-W)                       & 0.43m/1.62\degree  \\
%             +DFM (NeRF-Hist) & \textbf{0.15m}/\textbf{0.65\degree}  \\
%             \midrule
%             Direct-PN                            & 1.10m/4.25\degree  \\
%             Direct-PN+U                          & 1.41m/6.97\degree  \\
%             + NeRF-Hist                          & 0.72m/3.39\degree  \\
%             \bottomrule
%         \end{tabular}
%     }
%     % \vspace{-0.5cm}
% \end{wraptable}
